The Magic Number Conjecture for the $m=2$ amplituhedron and Parke-Taylor identities

The amplituhedron $A_{n,k,m}$ is a geometric object introduced in the context of scattering amplitudes in $N=4$ super Yang Mills. It generalizes the positive Grassmannian (when $n=k+m$), cyclic polytopes (when $k=1$), and the bounded complex of the cyclic hyperplane arrangement (when $m=1$). Of substantial interest are the tilings of the amplituhedron, which are analogous to triangulations of a polytope. Karp, Williams and Zhang (2020) observed that the known tilings of $A_{n,k,2}$ have cardinality ${n-2 \choose k}$ and the known tilings of $A_{n,k,4}$ have cardinality the Narayana number $\frac{1}{n-3}{n-3 \choose k+1}{n-3 \choose k}$; generalizing these observations, they conjectured that for even $m$ the tilings of $A_{n, k,m}$ have cardinality the MacMahon number, the number of plane partitions which fit inside a $k \times (n-k-m) \times \frac{m}{2}$ box. We refer to this prediction as the `Magic Number Conjecture'. In this paper we prove the Magic Number Conjecture for the $m=2$ amplituhedron: that is, we show that each tiling of $A_{n,k,2}$ has cardinality ${n-2 \choose k}$. We prove this by showing that all positroid tilings of the hypersimplex $\Delta_{k+1,n}$ have cardinality ${n-2 \choose k}$, then applying T-duality. In addition, we give combinatorial necessary conditions for tiles to form a tiling of $A_{n,k,2}$; we give volume formulas for Parke-Taylor polytopes and certain positroid polytopes in terms of circular extensions of cyclic partial orders; and we prove new variants of the classical Parke-Taylor identities.

==> abstract.tex <==
The \emph{amplituhedron} $\mathcal{A}_{n,k,m}(Z)$ is the
image of the
positive Grassmannian $\Gr_{k,n}^{\geq 0}$ under the
 map $\tilde{Z}: \Gr_{k,n}^{\geq 0} \to \Gr_{k,k+m}$ induced by a positive linear map 
$Z:\R^n \to \R^{k+m}$.
It was originally introduced in physics in order to give a 
geometric interpretation of 
scattering amplitudes.
More specifically, one 
can compute scattering amplitudes in $\mathcal{N}=4$ SYM 
by `tiling' the $m=4$ amplituhedron $\A_{n,k,4}(Z)$ --- 
that is, decomposing the amplituhedron into 
`tiles' (closures of images of $4k$-dimensional cells of $\Gr_{k,n}^{\geq 0}$
on which $\tilde{Z}$ is injective) --- and summing the `volumes' of the tiles.
In this article we prove the two main conjectures about 
 the $m=4$ amplituhedron.
We prove 
the \emph{BCFW tiling conjecture}, which says that any way of iterating the BCFW recurrence
gives rise to a tiling of the amplituhedron~$\A_{n,k,4}(Z)$.
And we prove 
the \emph{cluster adjacency conjecture} for BCFW tiles of $\A_{n,k,4}(Z)$, which says that
 facets of tiles are cut out by collections of compatible cluster variables 
for $\Gr_{4,n}$.  
We also show that each BCFW tile is the 
subset of $\Gr_{k, k+4}$ where certain cluster variables have particular signs.
Along the way we construct many explicit seeds for the 
$\Gr_{4,n}$ comprised of 
high-degree cluster variables, which may be of independent interest in the study of 
cluster algebras.


